Tensor Normal Training for Deep Learning Models

Despite the predominant use of first-order methods for training deep learning models, second-order methods, and in particular, natural gradient methods, remain of interest because of their potential for accelerating training through the use of curvature information. Several methods with non-diagonal preconditioning matrices, including KFAC, Shampoo, and K-BFGS, have been proposed and shown to be effective. Based on the so-called tensor normal (TN) distribution, we propose and analyze a brand new approximate natural gradient method, Tensor Normal Training (TNT), which like Shampoo, only requires knowledge of the shape of the training parameters. By approximating the probabilistically based Fisher matrix, as opposed to the empirical Fisher matrix, our method uses the block-wise covariance of the sampling based gradient as the pre-conditioning matrix. Moreover, the assumption that the sampling-based (tensor) gradient follows a TN distribution, ensures that its covariance has a Kronecker separable structure, which leads to a tractable approximation to the Fisher matrix. Consequently, TNT's memory requirements and per-iteration computational costs are only slightly higher than those for first-order methods. In our experiments, TNT exhibited superior optimization performance to state-of-the-art first-order methods, and comparable optimization performance to the state-of-the-art second-order methods KFAC and Shampoo. Moreover, TNT demonstrated its ability to generalize as well as first-order methods, while using fewer epochs.

==> sections/shampoo.tex <==


\subsection{order-2 tensor}
\label{sec_5}

We use the same notations as in \cite{gupta2018shampoo}. By (2) of \cite{gupta2018shampoo}, the preconditioning matrix is 
$$H_t = L_t^{1/4} \otimes R_t^{1/4}.$$
On the other hand, we know that the "ideal" preconditioning matrix (e.g. see GGT (\cite{agarwal2018case})) is
$$\left( E[g_t g_t^\top] \right)^{1/2},$$

\clarify{change $g_t$ to $\widehat{g}_t$ to denote gradient}

where the term inside $()$ can be viewed as the empirical Fisher matrix and the term $1/2$ comes naturally from Adagrad (\cite{duchi2011adaptive}). 

In order to justify Shampoo, we'd like to show that the following approximation is reasonable:
\begin{align}
\nonumber
H_t = & L_t^{1/4} \otimes R_t^{1/4} \approx \left( E[g_t g_t^\top] \right)^{1/2}
% \\
% \nonumber
% \Leftrightarrow & \left( L_t^{1/4} \otimes R_t^{1/4} \right)^2 \approx E[g_t g_t^\top]
% \\
% \nonumber
% \Leftrightarrow & L_t^{1/2} \otimes R_t^{1/2} \approx E[g_t g_t^\top]
% \\
% \nonumber
% \Leftrightarrow & \left( L_t^{1/2} \otimes R_t^{1/2} \right)^2 \approx \left( E[g_t g_t^\top] \right)^2
\\
\label{eq_1}
\Leftrightarrow & L_t \otimes R_t \approx E[g_t g_t^\top g_t g_t^\top]
\\
\nonumber
& \text{(we {\bf assume} that $\left( E[g_t g_t^\top] \right)^2 = E[g_t g_t^\top g_t g_t^\top]$)}
\end{align} 

% \addthis{
% the derivation in (1) could simply be stated as (ignoring the subscript t and using @ for K-product)) 
% $L^{1/4} @ R^{1/4} = (E[gg^T)]^{1/2} <=> L @ R = (E[gg^T])^2 $
% followed by the approx that the $E[G]^2 = E[G^2]$.
% }

Now we'd like to examine the LHS and RHS of the above formula under the {\bf assumption} that $G_t = g_t a_t^\top$, which is true for a fully-connected neural network. First,
\begin{align*}
    L_t = E[G_t G_t^\top]
    = E[g_t a_t^\top (g_t a_t^\top)^\top]
    = E[g_t a_t^\top a_t g_t^\top]
    = E[(a_t^\top a_t) (g_t g_t^\top)]
\end{align*}
Similarly,
\begin{align*}
    R_t = E[G_t^\top G_t]
    = E[(g_t a_t^\top)^\top g_t a_t^\top]
    = E[a_t g_t^\top g_t a_t^\top]
    = E[(g_t^\top g_t) (a_t a_t^\top)]
\end{align*}
On the other hand,
\begin{align*}
    & \widehat{g}_t = \text{vec}(G_t) = \text{vec}(g_t a_t^\top) = a_t \otimes g_t
    \\
    & \widehat{g}_t^\top \widehat{g}_t = (a_t \otimes g_t)^\top (a_t \otimes g_t)
    = (a_t^\top \otimes g_t^\top) (a_t \otimes g_t)
    = (a_t^\top a_t) \otimes (g_t^\top g_t)
    = (a_t^\top a_t) (g_t^\top g_t)
    \\
    & \widehat{g}_t \widehat{g}_t^\top = (a_t \otimes g_t) (a_t \otimes g_t)^\top
    = (a_t \otimes g_t) (a_t^\top \otimes g_t^\top)
    = (a_t a_t^\top) \otimes (g_t g_t^\top)
\end{align*}
Hence,
\begin{align*}
    & E[g_t g_t^\top g_t g_t^\top]
    = E[(g_t^\top g_t) (g_t g_t^\top)]
    = E[(a_t^\top a_t) (g_t^\top g_t) \left( (a_t a_t^\top) \otimes (g_t g_t^\top) \right)]
    \\
    & = E[ \left( (g_t^\top g_t) (a_t a_t^\top) \right) \otimes \left( (a_t^\top a_t) (g_t g_t^\top) \right) ]
    \\
    & \approx E[ (g_t^\top g_t) (a_t a_t^\top) ] \otimes E[ (a_t^\top a_t) (g_t g_t^\top) ]
    = R_t \otimes L_t
\end{align*}

\addthis{In the above, we showed our final {\bf approximation/assumption}. Also note that we use the fact that $k(A \otimes B) = (kA) \otimes B = A \otimes (kB)$
for any scalar $k$.}

% Thus, (\ref{eq_1}) is equivalent to
% \begin{align*}
%     E[(a_t^\top a_t) (g_t g_t^\top)] \otimes E[(g_t^\top g_t) (a_t a_t^\top)] \approx E[(a_t^\top a_t) (g_t^\top g_t) \left( (a_t a_t^\top) \otimes (g_t g_t^\top) \right)]
% \end{align*}
% which is our final {\bf approximation/assumption}. 

% \clarify{Just replace the rhs of the expression above it by $E[(g^Tg)aa^T @ (a^Ta) gg^T]$ as written on the top of p.14.}

\subsection{order-k tensor}

Similar as in Section \ref{sec_5}, the ideal preconditioning matrix is
\begin{align*}
    & \mathbb{E} [g g^\top]
    = \mathbb{E} [\text{vec}(G) \text{vec}(G)^\top]
    = \mathbb{E} [
    \begin{pmatrix}
    \text{vec}(G_1^1)^\top & \cdots & \text{vec}(G_{n_1}^1)^\top
    \end{pmatrix}^\top
    \begin{pmatrix}
    \text{vec}(G_1^1)^\top & \cdots & \text{vec}(G_{n_1}^1)^\top
    \end{pmatrix}
    ]
    \\
    = & \mathbb{E} \left[
    \begin{pmatrix}
    \text{vec}(G_1^1)
    \\ \vdots
    \\ \text{vec}(G_{n_1}^1)
    \end{pmatrix}
    \begin{pmatrix}
    \text{vec}(G_1^1)^\top & \cdots \text{vec}(G_{n_1}^1)^\top
    \end{pmatrix}
    \right]
    \\
    = & \mathbb{E} \left[
    \begin{pmatrix}
    \text{vec}(G_1^1) \text{vec}(G_1^1)^\top & \cdots & \text{vec}(G_1^1) \text{vec}(G_{n_1}^1)^\top
    \\ \vdots & \vdots & \vdots
    \\ \text{vec}(G_{n_1}^1) \text{vec}(G_1^1)^\top & \cdots & \text{vec}(G_{n_1}^1) \text{vec}(G_{n_1}^1)^\top
    \end{pmatrix}
    \right]
    \\
    = & 
    \begin{pmatrix}
    \mathbb{E} [ \text{vec}(G_1^1) \text{vec}(G_1^1)^\top ] & \cdots & \mathbb{E} [ \text{vec}(G_1^1) \text{vec}(G_{n_1}^1)^\top ]
    \\ \vdots & \vdots & \vdots
    \\ \mathbb{E} [ \text{vec}(G_{n_1}^1) \text{vec}(G_1^1)^\top ] & \cdots & \mathbb{E} [ \text{vec}(G_{n_1}^1) \text{vec}(G_{n_1}^1)^\top ]
    \end{pmatrix}
\end{align*}
Note that we omit the subscript $t$. 

We {\bf assume} that 
\begin{align*}
    \mathbb{E} [ \text{vec}(G_i^1) \text{vec}(G_j^1)^\top ]
    \approx H_{i,j}^1 \hat{G}^{-1},
\end{align*}
where $H_{i,j}^1$ is a scalar and $\hat{G}^{-1}$ is a matrix free of $i$ and $j$. Thus, 
\begin{align*}
    \mathbb{E} [g g^\top]
    \approx H^1 \otimes \hat{G}^{-1}
\end{align*}

$H_{i,j}^1$ can be viewed as the "overall magnitude" of $\mathbb{E} [ \text{vec}(G_i^1) \text{vec}(G_j^1)^\top ]$. To summarize the overall magnitude, we let
\begin{align*}
    H_{i,j}^1 = \mathbb{E} [ \text{vec}(G_i^1)^\top \text{vec}(G_j^1) ]
\end{align*}
Thus,
\begin{align*}
    H^1
    = \mathbb{E} \left[
    \begin{pmatrix}
    \text{vec}(G_1^1)^\top
    \\ \vdots
    \\ \text{vec}(G_{n_1}^1)^\top
    \end{pmatrix}
    \begin{pmatrix}
    \text{vec}(G_1^1) & \cdots \text{vec}(G_{n_1}^1)
    \end{pmatrix}
    \right]
    = \mathbb{E} \left[
    \text{mat}_1 (G)
    \text{mat}_1 (G)^\top
    \right]
    = \mathbb{E} [ G^{(1)} ]
\end{align*}

\subsection{Shampoo vs KFAC}

We {\bf assume} that the model is a fully-connected neural network. As shown in \cite{martens2015optimizing}, the Fisher (or empirical Fisher) matrix of a layer is
\begin{align*}
    \mathbb{E} [\text{vec}(G) \text{vec}(G)^\top] = \mathbb{E} [(a a^\top) \otimes (g g^\top)]
\end{align*}
We'd like to compare Shampoo and KFAC in terms of how they approximate the Fisher matrix. 

\begin{itemize}
    \item KFAC:
    
    KFAC approximates the Fisher matrix by $\mathbb{E} [(a a^\top)] \otimes \mathbb{E} [(g g^\top)]$. 
    
    \item Shampoo:
    
    We consider two different cases where either a individual stochastic gradient or a mini-batch stochastic gradient is processed in an iteration. 
    
    \begin{itemize}
        \item 
        In the case of individual stochastic gradient,
    \begin{align*}
        & G G^\top = (g a^\top) (g a^\top)^\top
        = g a^\top a g^\top
        = (a^\top a) (g g^\top)
        \\
        \Rightarrow
        & L = \mathbb{E} [G G^\top]
        = \mathbb{E} [(a^\top a) (g g^\top)]
    \end{align*}
    Similarly, 
    \begin{align*}
        R = \mathbb{E} [G^\top G]
        = \mathbb{E} [(g^\top g) (a a^\top)]
    \end{align*}
    Finally, the Fisher matrix is approximated by $L^{1/2} \otimes R^{1/2}$. 
    
        \item
        In the case of mini-batch stochastic gradient,
    \begin{align*}
        G G^\top
        = (\frac{1}{N} \sum_{i=1}^N g_i a_i^T) (\frac{1}{N} \sum_{i=1}^N g_i a_i^T)^\top
        = \frac{1}{N^2} \sum_{i,j} (a_i^\top a_j) g_i g_j^\top
    \end{align*}
    In this case, it is harder to interpret $L$ and $R$. 
    \end{itemize}
    
    
    
\end{itemize}


